A global proof of the homological excess intersection formula

We provide a novel proof of the homological excess intersection formula for local complete intersections. The novelty is that the proof makes use of global morphisms comparing the intersections to a self intersection.

==> Prelims/Koszul/K-alg.tex <==
We begin with an aside on Koszul complexes. Most of the results here can be found in \cite{Matsumura} for the algebraic case or \cite{F-L} for the geometric case. 

\subsubsection{Koszul complexes in commutative algebra}\label{K-alg}

 Let $R$ be a ring and let $s: M \rightarrow R$ be a map of free $R$-modules. 
 
 \begin{definition}
 The \textit{Koszul complex} of $(M,s)$ over $R$ is the complex of $R$-modules concentrated in negative degree whose terms are $K^{-p}(M,s) = \bigwedge_R^p M$ for $p \geq 0$. The differentail of this complex is given by
 \[m_1\wedge \dots \wedge m_p \mapsto \sum_{i =1}^p (-1)^i s(m_i) (m_1\wedge \dots \wedge\widehat {m_i} \wedge\dots \wedge m_p)\]
 where $\widehat{m_i}$ means to omit the $m_i$ term from the exterior product.
 \end{definition}
 \noindent
% (1_R \wedge s \wedge 1 \wedge \dots \wedge 1) \circ (s \wedge 1 \wedge \dots \wedge 1).
We write $K^\bullet(R^r,s) =: K^\bullet(f_1,\dots,f_r)$ where $f_i = s(e_i)$ is the image of the $i^{th}$ standard generator. 
\par
Koszul complexes are nicely behaved with respect to tensor products;
\begin{proposition}
Suppose we have two linear maps $s: E \rightarrow R, t : F \rightarrow R$ of free modules of finite rank into $R$. Then we have the identification 
\[K^\bullet(E,s)\otimes K^\bullet(F,t) \cong K^\bullet(E\oplus F,s\oplus t).\]
In particular  if $F \cong R$, we get
\[K^\bullet(E\oplus R,s\oplus t) \cong Cone(t:K^\bullet(E,s)\rightarrow K^\bullet(E,s)).\]
\end{proposition}
We are interested in the cohomologies of these complexes. In particular the following is a well known criterion for a Koszul complex $K^\bullet(\underline{f})$ to be a resolution of $R/(f_1,\dots,f_n)$; 

\begin{definition}
We say a sequence of elements $f_1,\dots, f_n \in R$ form a regular sequence in $R$ if $f_1$ is not a zero-divisor in $R$ and for each $i > 1$, $f_i$ is not a zero-divisor in $R/(f_1,\dots,f_{i-1})R.$
\end{definition}


\begin{proposition}
Let $f_1,\dots,f_n$ form a regular sequence in a ring $R$. Then $h^i(K^\bullet(f_1,\dots,f_n)) = 0$ for all $i \neq {-1}$ and $h^0(K^\bullet(f_1,\dots,f_n)) = R/(f_1,\dots,f_n)$, i.e. $K^\bullet(f_1,\dots,f_n)$ is a free resolution of $R/(f_1,\dots,f_n).$
\end{proposition}

In general the converse does not hold (see \cite{Kabele}), but for instance in Noetherian local rings with $f_1,\dots, f_n$ in the maximal ideal it does \cite{Matsumura}. 
%\begin{proof}
%By induction. If $r = 1$, then since $f_1$ is not a zero-divisor in $R$ we can see that the homology of the complex
%\[
 %   \begin{tikzcd}
  %  K^\bullet(f_1) = 0 \arrow[r] &R \arrow[r,"f_1"] &R \arrow[r] &0\\
   % \end{tikzcd}
%\]
%is as desired. By Proposition 2.1.1 we can write
%\[K^\bullet(f_1,\dots,f_r) = Cone(f_r:K^\bullet(f_1,\dots,f_{r-1})\rightarrow K^\bullet(f_1,\dots,f_{r-1})).\]
%The upshot of viewing the Koszul complex as a cone is that we have a long exact sequence on cohomology 
%\[\dots \rightarrow H^j(K_{r-1}) \rightarrow H^j(K_{r-1}) \rightarrow H^j(K_{r}) \rightarrow H^{j-1}(K_{r-1}) \rightarrow \dots\]
%where $K_r$ is shorthand notation for $K^\bullet(f_1,\dots,f_r).$ By the inductive hypothesis, the only non-zero part of this exact sequence is
%\[0 \rightarrow H^1(K_r) \rightarrow H^0(K_{r-1}) \rightarrow H^0(K_{r-1}) \rightarrow H^0(K_r) \rightarrow 0\]
%where $H^0(K_{r-1}) \rightarrow H^0(K_{r-1})$ is multiplication by $f_r.$ Since $H^0(K_{r-1}) = R/(f_1,\dots,f_{r-1})R$ and $f_r$ is not a zero-divisor in this quotient ring, we see that $H^1(K_r) = 0$ and also that $H^0(K_r) = (R/(f_1,\dots,f_{r-1}))/(f_r) = R/(f_1,\dots,f_r)$ as desired.
%\end{proof}





==> Prelims/Lci/main.tex <==



%\begin{proposition}
%Let $X$ be a nonsingular variety over a field $k$. Let $Y_1,\dots,Y_n$ be local complete intersection subvarieties of $X$ of codimensions $c_1,\dots,c_n$ respectively. If $Z = \bigcap Y_i$ has codimension $c = \sum c_i$ (i.e. the $Y_i$ intersect dimensionally transversally), then $Z$ is a local complete intersection.  
%\end{proposition}

%\begin{proof}
%A local complete intersection has ideal sheaf locally generated by a number of elements equal to its codimension. We have $\mathcal{I}_Z = \sum_{i=1}^n \mathcal{I}_{Y_i}$. Since each $Y_i$ is a local complete intersection, $\mathcal{I}_{Y_i}$ is locally generated by $c_i$ elements, and so sufficiently locally, $\mathcal{I}_Z$ is generated by $\sum_{i =1}^n c_i = c$ elements. By assumption, this is the codimension of $Z$ and so $Z$ is a local complete intersection. 
%\end{proof}



==> TODO.tex <==
%% change all of your h^{-q} to H^{-q}...
